Learning to Reach Goals via Iterated Supervised Learning

Current reinforcement learning (RL) algorithms can be brittle and difficult to use, especially when learning goal-reaching behaviors from sparse rewards. Although supervised imitation learning provides a simple and stable alternative, it requires access to demonstrations from a human supervisor. In this paper, we study RL algorithms that use imitation learning to acquire goal reaching policies from scratch, without the need for expert demonstrations or a value function. In lieu of demonstrations, we leverage the property that any trajectory is a successful demonstration for reaching the final state in that same trajectory. We propose a simple algorithm in which an agent continually relabels and imitates the trajectories it generates to progressively learn goal-reaching behaviors from scratch. Each iteration, the agent collects new trajectories using the latest policy, and maximizes the likelihood of the actions along these trajectories under the goal that was actually reached, so as to improve the policy. We formally show that this iterated supervised learning procedure optimizes a bound on the RL objective, derive performance bounds of the learned policy, and empirically demonstrate improved goal-reaching performance and robustness over current RL algorithms in several benchmark tasks.

==> commands.tex <==
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{amsthm}
\usepackage{mathtools}
\usepackage{natbib}
\usepackage{enumerate}
\usepackage{tikz}
\usepackage{graphicx}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{conjecture}{Conjecture}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollaryp}{Corollary}[proposition]
\newtheorem{definition}{Definition}[section]

\newcommand{\TODO}[1]{\textcolor{red}{TODO: #1}}

\newcommand{\citemissing}{\textcolor{red}{(cite?)}}

\DeclarePairedDelimiter\abs{\lvert}{\rvert}%
\DeclarePairedDelimiter\norm{\lVert}{\rVert}%
\DeclarePairedDelimiter\ceil{\lceil}{\rceil}
\DeclarePairedDelimiter\floor{\lfloor}{\rfloor}

\newcommand{\normt}[1]{\left\lVert#1\right\rVert_2}
\newcommand{\normm}[1]{\left\lVert#1\right\rVert}
\newcommand{\norminf}[1]{\left\lVert#1\right\rVert_\infty}
\newcommand{\normtt}[1]{\left\lVert#1\right\rVert^2_2}
\newcommand{\Ainv}{A^{-1}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\fourth}{\frac{1}{4}}
\newcommand{\xsum}{x^{sum}}
\newcommand{\ysum}{y^{sum}}
\newcommand{\vect}[1]{\overrightafrrow{\textbf{#1}}}
\newcommand{\phat}{\hat{p}}
\newcommand{\KL}[2]{D_{KL}(#1||#2)}
\newcommand{\TV}[2]{D_{TV}(#1||#2)}
\newcommand{\ind}[1]{1[#1]}
\newcommand{\pardiv}[1]{\frac{\partial}{\partial #1}}
\newcommand{\parHess}[1]{\frac{\partial^2}{\partial #1 ^2}}
\newcommand{\Xhat}{{\hat{X}}}
\newcommand{\xhat}{{\hat{x}}}
\newcommand{\Qhalf}{Q^{\frac{1}{2}}}
\newcommand{\Qneghalf}{Q^{-\frac{1}{2}}}
\newcommand{\defeq}{\mathrel{\stackrel{\makebox[0pt]{\mbox{\normalfont\tiny def}}}{=}}}

\newcommand{\lambdabar}{{\bar{\lambda}}}
\newcommand{\argmax}[1]{\underset{#1}{\textrm{argmax}}}
\newcommand{\argmin}[1]{\underset{#1}{\textrm{argmin}}}
\newcommand{\grad}[1]{\nabla{#1}}
\newcommand{\innerp}[2]{\langle{#1,#2}\rangle}
\newcommand{\Hess}[1]{\nabla^2{#1}}
\newcommand{\EXP}[1]{\text{exp}\{#1\}}

\newcommand{\Rmax}{R_{\textrm{max}}}
\newcommand{\data}[1]{\bar{#1}}
\newcommand{\datapi}{{\bar{\pi}}}
\newcommand{\newpi}{\pi^\textrm{new}}
\newcommand{\Kret}[2]{\eta^{#1//#2}_K}
\newcommand{\Khatret}[2]{\hat{\eta}^{#1//#2}_K}
\newcommand{\Kprobsa}[2]{p^{#1//#2, K}}
\newcommand{\epsmodel}{\epsilon_m}
\newcommand{\epspi}{\epsilon_\pi}




==> text/broader_impacts.tex <==
\section{Broader Impact Statement}
Despite widespread applicability in domains ranging from robotics to healthcare, reinforcement learning algorithms have seen somewhat limited adoption because of challenges in applying the algorithms quickly and easily to a variety of different problems. Typical RL algorithms can often be unstable, brittle to choices of hyperparameters, and hard to use and modify without significant expertise or prior knowledge. In this work, we attempted to design a simple, stable, and robust algorithm for learning control policies that can be easily used without the need for complex RL machinery such as value functions. GCSL optimizes a clearly defined supervised learning objective, is robust to hyperparameter changes, and perhaps most importantly, can be implemented with just a few lines of code. Developing and focusing on RL algorithms that are simpler to use and apply to new problems, like GCSL, would greatly incentivize adoption of RL for solving real-world problems. We hope that this line of research helps RL grow from being a niche tool used only by domain experts, potentially towards widespread adoption across a variety of problem domains and end users. While this paper studies these situations in simulation, we hope it can serve as a building block for enabling discovery of such behaviors in the real world as well.

Our work focuses specifically on RL for goal-reaching. While at first this may seem narrow, in fact goal-reaching behavior constitutes a large number of practical RL problems. In industrial robotics, picking and placing objects can be cast as reaching goals; in autonomous driving, navigation as goal-reaching; and in general, sparse-reward problems in RL can be cast as the solution to a sequence of goal-reaching problems. Our empirical results demonstrated that GCSL to be successful at acquiring goal-reaching behaviors on many practical tasks in simulation, including a simulated Sawyer robot pushing blocks and opening doors, and a simulated claw robot rotating valves.

From a broader perspective, making autonomous decision making agents easier to use and more ubiquitous can have both beneficial and harmful impacts on society. For many domains, where deploying human resources can be dangerous, challenging or extremely expensive, widespread use of learning algorithms such as GCSL would allow for positive effects both economically and by avoiding putting human lives at risk. However, replacing human resources by automated decision making systems naturally can have negative societal impacts in how it impacts employment opportunities and affect the livelihoods of many, besides the concerns of how these technologies may be misused by malicious actors. To this end, we need to better understand which problems actually stand to benefit from RL algorithms with minimal safety or privacy concerns and which problems can be tackled by other techniques. 

